On the Intrinsic and Extrinsic Fairness Evaluation Metrics for Contextualized Language Representations

Multiple metrics have been introduced to measure fairness in various natural language processing tasks. These metrics can be roughly categorized into two categories: 1) \emph{extrinsic metrics} for evaluating fairness in downstream applications and 2) \emph{intrinsic metrics} for estimating fairness in upstream contextualized language representation models. In this paper, we conduct an extensive correlation study between intrinsic and extrinsic metrics across bias notions using 19 contextualized language models. We find that intrinsic and extrinsic metrics do not necessarily correlate in their original setting, even when correcting for metric misalignments, noise in evaluation datasets, and confounding factors such as experiment configuration for extrinsic metrics. %al

==> sections/archive.tex <==

% \begin{table*}[ht]
% \centering
% \begin{tabular}{|l|c|c|c|c|c|c|}
% \hline
% & \multicolumn{2}{c|}{Gender} & \multicolumn{2}{c|}{Race} & \multicolumn{2}{c|}{Religion}\\
% \hline
% & \Mceat& \Mtceat & \Mceat& \Mtceat &\Mceat & \Mtceat\\ 
% \hline
% \Mtoxdetect &  -0.120 & 0.040  & -0.056 & 0.078 & 0.279  & 0.415 \\ \hline
% \Mhate  &  -0.119 & 0.165  & -0.046 & 0.486 & 0.231  & 0.434 \\ \hline
% \Mboldtox & 0.213 & \textbf{0.909}  & 0.405 & 0.409  & 0.194 & 0.556 \\ \hline
% \Mboldsent & -0.030 & -0.463 & \textbf{0.674} & -0.18   & 0.105 & 0.375  \\ \hline
% \end{tabular}
% \caption{\label{tab:tox_ablation_toxwords} Domain-level results. Results in bold are statistically significant.}
% \end{table*}


\begin{table}[t]
\small
\centering
\begin{tabular}{|l|c|c|c|}
\hline
& Gender & Race & Religion\\
\hline
&  \Mtceat & \Mtceat  & \Mtceat\\ 
\hline
\Mtoxdetect &   0.04   & 0.08   & 0.42 \\ \hline
\Mhate  &   0.17 & 0.49   & 0.43 \\ \hline
\Mboldtox  & \textbf{0.91} & 0.41   & 0.56 \\ \hline
\Mboldsent  & -0.46  & -0.18    & 0.38  \\ \hline
\end{tabular}
\caption{\small \label{tab:tox_ablation_toxwords} Domain-level results. Results in bold are statistically significant.}
\end{table}



There are many factors at play in fairness evaluation processes, such as quality of the testing data, choice of protected groups, and notion of bias measured.
In this section, we conduct careful analysis to explore why extrinsic and intrinsic metrics are not always correlated. 
% While in the experiments above, we follow the settings in the papers that introduce the metrics and datasets, to understand why we have unexpected correlation results, in this section we explore the impact of computing the proposed metrics outside the settings followed in those papers.
% In the above experiments, we simply follow the choices as in the metrics' original paper. 
% To understand why we have unexpected correlation results, 
% We carefully align these metrics on the notion of bias and target groups within each domain, as well as improve the quality of evaluation datasets. 

\subsection{Misalignment between metrics}
 In our main study, we use the original cast of the datasets and metrics. However, these metrics may have subtle misalignments in type of bias,  protected group, and characteristics of the underlying dataset. With this in mind, we perform the below ablation studies.

\paragraph{Misalignment on the notion of bias}
Among the toxicity metrics, the notion of bias are not consistent -- some measure sentiment (\Mceat, \Mlpbs, \Mboldsent) while others measure toxicity. 
Therefore, we recompute CEAT scores with toxicity word seeds, which we denote as \Mtceat. We manually pick 20 \emph{toxic} and 20 \emph{anti-toxic} words from the word clouds of the toxic and non-toxic labeled sentences in the JigsawToxicity dataset for \Mtceat. See \autoref{sec:tceat attributes} for the full list of the words.

% \subsubsection{Ablation Study: Aligning CEAT word sets with toxicity metrics}

% To test our hypothesis that the negative correlations between intrinsic metrics and BOLD toxicity are due to a mismatch of type of bias measured between the two, we  calculate \Mtceat, which uses toxic word sets as testing words for CEAT measurement. 

% We collect \emph{toxic} and \emph{anti-toxic} words from the JigsawToxicity dataset and use those words to recalculate the CEAT scores. We manually pick 20 \emph{toxic} and 20 \emph{anti-toxic} words from the word clouds of the toxic and non-toxic labeled sentences. See appendix for the full list of the words.


As seen in \autoref{tab:tox_ablation_toxwords}, we see that the correlations between the toxicity-related extrinsic metrics and \Mtceat are more positive than with \Mceat. This is in line with the expected result, though many of the correlation scores remain not statistically significant. 
We also note that \Mceat is better correlated with \Mboldsent than \Mtceat, except for religion.  
This supports our hypothesis that intrinsic and extrinsic metrics are more correlated when they have the same notion of bias.
% This supports our hypothesis that intrinsic and extrinsic metrics have more aligned testing data, which is testing words sets in this case, the two metrics will be more correlated. 

\paragraph{Misalignment on the protected groups}
Due to the limited number of overlapping protected groups (stereotype metrics only have four groups in common), we compute the domain-level variance scores for all protected groups contained in a dataset. However, this may introduce bias from groups in an intrinsic metric that is not present in an extrinsic metric, or vice versa. Thus in the ablation study, we pick the domain \emph{race} and recompute the correlation of \Mstereoset with \Mboldregard and \Mboldstereo with only overlapping protected groups\footnote{\Mstereoset does not have group Asian and White, so we use Japanese and Britain instead for these groups.}: White, Black, Hispanic, and Asian.


We find that the correlation of \Mstereoset with \Mboldregard raises from $-0.08$ to $0.19$ (p-value $0.56$). The correlation with \Mboldstereo increases from $-0.18$ to $0.08$ (p-value $0.80$). These metrics are more positively correlated with the aligned protected groups.


\paragraph{Misalignment on underlying dataset}
The dataset sources for BOLD and StereoSet are very different. \Mstereoset uses crowdworkers to generate testing data specifically to contain particular stereotypes. On the other hand, BOLD prompts are sourced from Wikipedia, which consist of more formal writing and is not directly engineered to probe for stereotypes. 

To align the stereotype metrics, we use data from the \Mstereoset intersentence dataset, which consists of a one-sentence context followed by a relevant stereotyped sentence, for BOLD metrics. Specifically, we use the context sentence for BOLD-like generation (see \autoref{sec:stereoset-bold-gen} for generation examples). We test \Mstereoset with the new \Mboldstereo on the \emph{race} domain and find that the correlation score increase from $-0.18$ to $0.02$ (p-value 0.98). 
This indicates that aligning the underlying dataset has a modest impact on improving correlation between metrics.

\subsection{Noisy Evaluation Datasets}
As pointed out in \citet{norweigen}, current stereotype datasets lack consistency in framing and data collection methodology, which leads to datasets that do not properly evaluate the intended notion of bias. We find evidence of bias in the BOLD dataset for religion prompts, specifically, prompts which already contain toxic and stereotyped content. 
We use the sentiment, regard, and toxicity classifier to filter out prompts that have higher polarity values, and recalculate the correlations of intrinsic metrics with BOLD-related extrinsic metrics on \emph{religion} domain. 
We find that scores for \Mceat and \Mboldsent increases to $0.11$, \Mstereoset and \Mboldstereo increases to $0.10$. 
This indicates that noisy datasets can affect the metrics. 

\subsection{Variation in Generation Metric Scores due to Experiment Configuration}

In our main study, we fix the sampling procedure for generation tasks in order to isolate the effect of varying language models in our correlation study without the confounding effect of varying generation procedures. 

However, generation fairness scores can be impacted by the hyper-parameter choice used during the language model fine-tuning (e.g. learning rate) or language model generation (e.g. decoding temperature).
Additionally, extrinsic metrics that use ML models (e.g. sentiment classifier) as part of metric computation can be impacted by the quality of such models.

% YADA: comment out for space. \citet{baldini_2021} report that different random initialization and dataset size for finetuning influence toxicity classification metrics.
We conduct two additional experiments, which demonstrate that sampling temperature has great impact on the sentiment level of the generations and the sentiment classifier is not robust to the noise in the generated texts, in which (i) we evaluate the impact of choosing a different decoding temperature on BOLD metrics and (ii) assess the impact of adding noise in generated outputs on sentiment classification. 

\textbf{Impact of sampling temperature on metrics} We feed five sample prompts (enlisted in Appendix X) from BOLD dataset to GPT-2 model and for each prompt, generate 100 sentences. We use two temperature settings (T = 0.5 and T = 1.0) and compute the average sentiment over the generated sentences. We observe that the proportion of negative sentiment assignment increases from 4.6\% to 15.6\% by just changing the temperature, and thus the generation quality and diversity.

\textbf{Impact of noise in generated outputs on sentiment classification}
We conduct a synthetic experiment where we either swap or delete words in $\sim 1400$ BOLD generations (examples shown in Appendix Y). We acknowledge that noise in real world may look different, however, the point of this study is just to test the robustness of classifier based metrics to invariant word substitutions and deletions. We present full results in Appendix Y and observe that the sentiment metrics, particularly in the case of deletions swing between values of 7.14\% to 4.46\%. This showcases that the extrinsic metrics are also a function of the robustness of the classifiers used to compute them, while intrinsic metrics are not impacted by the choice of such a classifier. 

These ablation studies highlight a limitation in lack of robustness of model-based generation metrics, which we encourage for future work. 

==> sections/method.tex <==

\yada{
\subsection{Models} 
For models, we run experiments on twelve models. We evaluate the intrinsic metrics and BOLD language generation on all models, however, we only evaluate toxicity classification on and RoBERTa. 

\subsection{Domains} 
For domains, we conduct this study on race, religion, and gender. The groups used are from \cite{https://aclanthology.org/2021.findings-acl.355.pdf}. The groups used for these domains in the datasets used are below.  
\begin{table}
    \centering
\begin{tabular}{ | m{4em} | m{2cm}| m{3cm} | } 
\hline
 Dataset & Domain & Annotated Groups \\

  \hline
  BOLD & Gender & Male, Female \\ 
  \hline
  BOLD & Race & European Americans, African Americans, Asian Americans, and Latino / Hispanic Americans \\ 
  \hline
  BOLD & Religion & Sikhism, Judaism, Islam, Hinduism, Christianity, Buddhism, and Atheism \\ 
  \hline
  StereoSet & Gender & Male, Female, Transgender, Other Gender \\ 
   \hline
  StereoSet & Race & 149 nationalities (i.e. German) \\ 
   \hline
  StereoSet & Religion & Christian, Muslim, Islam, Hindu \\
   \hline
  Jigsaw Toxicity & Gender & Male, Female \\ 
   \hline
  Jigsaw Toxicity & Race & White, Black, Asian, Latino \\ 
   \hline
  Jigsaw Toxicity & Religion & Christian, Jewish, Muslim, Hindu, Buddhism, Atheist \\
    \hline
\end{tabular}
\end{table}
We see that there is not an exact match in groups in domains, thus we take the groups that are contained in the intersection (highlighted in bold). 

\section{Method} 
To do a rigorous study on correlations between extrinsic and intrinsic metrics, we examine both domain-level and group level correlations. Domain-level metrics give a good understanding of how disparities between cohorts transfers between various tasks, while group level metrics give a good understanding of how bias characteristics for a particular group transfers across types of evaluation. 

}

==> sections/related.tex <==

Multiple work has examined the relationship between fairness metrics. From a societal and theoretical perspective, researchers have explored the relationship between group and individual fairness notions and metrics \cite{Binns2020OnTA}. While some prior work has empirically shown that improving fairness at the word embedding level has downstream impact on downstream fairness \cite{biasbios}, more recent work has shown that there are no consistent correlations between intrinsic and extrinsic fairness metrics \cite{intrinsicvsextrinsic}.  \citet{WEFE} created WEFE, an evaluation framework for word-embedding related fairness metrics, and showed that gender bias within existing embedding-based fairness metrics were correlated. From a societal standpoint,  \citet{norweigen} critique the pitfalls of current fairness metrics and benchmarks, and the lack of consistency in framing and data collection methodology for fairness evaluation datasets. 
    
The most similar work to ours is \cite{intrinsicvsextrinsic}, however, while they focus on static word embeddings and gender bias, we do an extensive study on contextualized embeddings, and expand to other domains. 

